PCA of probability measures: Sparse and Dense sampling regimes

A common approach to perform PCA on probability measures is to embed them into a Hilbert space where standard functional PCA techniques apply. While convergence rates for estimating the embedding of a single measure from $m$ samples are well understood, the literature has not addressed the setting involving multiple measures. In this paper, we study PCA in a double asymptotic regime where $n$ probability measures are observed, each through $m$ samples. We derive convergence rates of the form $n^{-1/2} + m^{-\alpha}$ for the empirical covariance operator and the PCA excess risk, where $\alpha>0$ depends on the chosen embedding. This characterizes the relationship between the number $n$ of measures and the number $m$ of samples per measure, revealing a sparse (small $m$) to dense (large $m$) transition in the convergence behavior. Moreover, we prove that the dense-regime rate is minimax optimal for the empirical covariance error. Our numerical experiments validate these theoretical rates and demonstrate that appropriate subsampling preserves PCA accuracy while reducing computational cost.

==> brenier.tex <==
\section{Brenier}

From the LOT embedding, one can also derive the \emph{Brenier embedding}, which has not yet been thoroughly studied.

\subsubsection{Brenier embedding}

Recall from Brenier's theorem \ref{th:brenier} that the Monge map $T_{\mu}$ is characterized as the gradient of a convex function $\varphi_{\mu}$. The Brenier embedding consists in using $\varphi_{\mu}$ rather than $T_{\mu}$.

\begin{align*}
    \Phi^{\mathrm{Br}} : \mathcal{M}(\mathcal{X}) & \rightarrow L^2(\rho)                                 \\
    \mu                                           & \rightarrow \varphi_{\mu} - \mathrm{Id}^T \mathrm{Id}
\end{align*}

The Brenier embedding was proposed
in Remark 3.2 of \cite{merigot2020quantitative}, but was to our knowledge never studied in practice. As for the LOT embedding, the Brenier embedding defines a distance between probability measures:

$$
    W_{2,\mathrm{Br}}^2(\mu,\nu) = \|\varphi_{\mu} - \varphi_{\nu}\|_{L^2(\rho)}^2.
$$

The Brenier embedding may ultimately prove advantageous as \cite{merigot2020quantitative} show that the exponents in the quantitative stability bounds $W_{2,\mathrm{Br}}(\mu,\nu) \leq CW^q_{2}(\mu,\nu)$ could be slightly better than for the LOT embedding. In other words, the Brenier embedding could yield a better approximation of the Wasserstein distance than the LOT embedding.


\subsection{Brenier embedding}

The Brenier embedding with reference measure $\rho$ of a probability measure $\mu$ is:

$$
    \Phi^{\mathrm{Br}}(\mu) = \varphi_{\mu} - \mathrm{Id}^T\mathrm{Id} \in L^2(\rho).
$$

In the Gaussian case, with $\rho = \mathcal{N}(0,I_d)$ and $\mu = \mathcal{N}(\bs{b},\bs{S})$, the Brenier embedding boils down to:

$$
    \Phi^{\mathrm{Br}}(\mu)(x) = x^T (\bs{S}^{1/2}-I_d)x + \bs{b}^Tx.
$$

\begin{proposition}\label{prop:brenier_eigfunc}
    If $\bs{\mu} = \mathcal{N}(\bs{b},~ \bs{\sigma} I_d)$, then the covariance operator of $\Phi^{\mathrm{Br}}(\bs{\mu})$ admits the following eigendecomposition
    \begin{itemize}
        \item $\forall 1\leq i \leq d, \forall x\in\mathcal{X}, f_i(x) = x_i $ with corresponding eigenvalue $\mathbb{E}[b_i^2].$
        \item Let $c_1,\cdots,c_d$ be the eigenvectors of the matrix $(\mathbb{E}[s_1]-1)(2I_d+11^T)$ with corresponding eigenvalues $\lambda_1,\cdots,\lambda_d$. Define $\forall 1\leq i\leq d, g_i(x) = \sum_{k=1}^d c_{ik} x_k^2$.If $\forall 1\leq i\leq d$, $\mathbb{E}[s_i] = \mathbb{E}[s_1]$, then  $\forall 1\leq i \leq d$, $\overline{g}_i(x) = \frac{g_i(x)}{\|g_i\|_{L^2(\rho)}}$ is an eigenfunction of $\Sigma$ with corresponding eigenvalue $\lambda_i$.
    \end{itemize}
\end{proposition}

One can observe that $\nabla f_i(x) = e_i$, which is an eigenfunction of the LOT embedding. This seems similar to the fact that the LOT embedding is the gradient of the Brener embedding.

\begin{proof}
    Let $f_i(x) = x_i$ and  $g_i(x) = \sum\limits_{k=1}^d x_k^2$. Denoting $\forall 1\leq i\leq d,\overline{\bs{s}}_i = \sqrt{\bs{s}}_i^{1/2}-1$, we can rewrite the embedding as:

    \begin{align*}
        \Phi^{\mathrm{Br}}(\bs{\mu})(x) &= \sum\limits_{i=1}^d \bs{b}_i f_i(x) + \overline{\bs{\sigma}} g\\
    \end{align*}

    We can now compute the covariance operator $\Sigma$ of the random variable $\Phi^{\mathrm{Br}}(\bs{\mu})$.

    \begin{align*}
    \Sigma &= \mathbb{E} \Bigl[\Phi^{\mathrm{Br}}(\bs{\mu}) \otimes \Phi^{\mathrm{Br}}(\bs{\mu})\Bigr]- \mathbb{E}\Bigl[\Phi^{\mathrm{Br}}(\bs{\mu})\Bigr] \otimes \mathbb{E}\Bigl[\Phi^{\mathrm{Br}}(\bs{\mu})\Bigr]\\
    &= \mathbb{E}\Bigl[\bigl(\sum\limits_{i=1}^d \bs{b}_i f_i + \overline{\bs{\sigma}} g\bigr) \otimes \bigl(\sum\limits_{j=1}^d \bs{b}_j f_j + \overline{\bs{\sigma}} g\bigr)\Bigr] - \mathbb{E}\Bigl[\sum\limits_{i=1}^d \bs{b}_i f_i + \overline{\bs{\sigma}} g\Bigr] \otimes \mathbb{E}\Bigl[\sum\limits_{j=1}^d \bs{b}_j f_j + \overline{\bs{\sigma}} g\Bigr]\\
    &= \sum\limits_{i=1}^d \mathbb{E}[\bs{b}_i^2] f_i \otimes f_i +  \mathbb{E}[\overline{\bs{\sigma}}^2] g \otimes g - \sum\limits_{i=1}^d \mathbb{E}[\bs{b}_i]^2 f_i \otimes f_i - \mathbb{E}[\overline{\bs{\sigma}}]^2 g \otimes g\\
    &= \sum\limits_{i=1}^d \mathrm{Var}(\bs{b}_i) f_i \otimes f_i + \mathrm{Var}(\overline{\bs{\sigma}}) g \otimes g\\
    \end{align*}
    \end{proof}


\subsection{Brenier embedding}

We follow the setting of the previous section and consider two absolutely continuous probability measures $\rho$ and $\mu$ supported on $\mathcal{X}\subset\mathbb{R}^d$ with respective densities $f$ and $g$. We denote $\varphi_0$ the Brenier potential between $\rho$ and $\mu$ such that $\nabla \varphi_0$ is the OT map between $\rho$ and $\mu$. We observe two sets of $m$ samples from $\rho$ and $\mu$, $X_1,\cdots, X_m \overset{i.i.d.}{\sim} \rho$ and $Y_1,\cdots, Y_m \overset{i.i.d.}{\sim} \mu$. From these samples, we consider estimators $\hat{\varphi}$ of $\varphi_0$ and study the rate of convergence under the loss function

$$
\mathbb{E}\|\hat{\varphi} - \varphi_0\|_{L^2(\rho)}.
$$

In \cite{gunsilius2022convergence}, the estimator for $\varphi_0$ is chosen as a smoothed plug-in estimator, that is the solution to:

$$
\argmin\limits_{\varphi \in C(\mathcal{X})} \int_{\mathcal{X}} \varphi(x)\mathrm{d} \rho_m * K_{h_m}(x) + \int_{\mathcal{X}} \varphi^*(y)\mathrm{d} \mu_m * K_{h'_m}(y),
$$

where $\rho_m * K_{h_m}(x) = \frac{1}{mh_m^d}\sum_{j=1}^m K(\frac{X_j - x}{h_n})$ and $K(\frac{X_i-x}{h_n}) = K'(\frac{X_{i1} - x_1}{h_n})\cdots K'(\frac{X_{id} -x_d}{h_n})$ is a product smoothing kernel with $h_n$ denoting the bandwidth.


\begin{theorem}[Corollary 1 in \cite{gunsilius2022convergence}]
We assume $\mathcal{X}$ is compact and convex and the densities $f$ and $g$ are bounded above and below. We also suppose that $f$ and $g$ are $s$-Hölder continuous on every compact subset of the interior of $\mathcal{X}$. Finally, let the kernel $K$ be non-negative, of second order, and the bandwidths $h_m,h_m'>0$ verify $h_m^2n^{1/2} \rightarrow 0$ and $(h_m')^2n^{1/2} \rightarrow 0$. Under the normalization $\int_{\mathcal{X}} \varphi(x)\mathrm{d}\rho(x) = 0$, we have that:


\[
\mathbb{E}\|\hat{\varphi} - \varphi_0\|_{L^2(\rho)} \lesssim r_m \qquad r_m = \begin{cases}
m^{-\frac{s}{2s+d}}, & s > d/2, \\
 \frac{\sqrt{\log m}}{m^{1/4}}, & s = d/2, \\
m^{-\frac{1}{s(2s+d)}}, & s < d/2.
\end{cases}
\]
\end{theorem}


\subsubsection{Brenier embedding}

\begin{lemma}\label{lemma:hypothesis_separation_brenier}
For $k\in\{1,2\}$, let $\Sigma^{(k)}$ be the covariance operator of the random embedding $\Phi^{\mathrm{Br}}(\bs{\mu}^{(k)})$. If $R\geq 4(d^2+2d)$ and if

\begin{equation}\label{eq:s_constraint}
1\leq s \leq \sqrt{\frac{R}{d^2+2d}} -1,
\end{equation}

then, $\bs{\mu}^{(k)} \in \mathcal{D}(R)$.  Furthermore,

\begin{equation}\label{eq:cov_operators_diff}
\|\Sigma^{(1)} - \Sigma^{(2)}\|_{\mathrm{HS}} \geq 2 C^{\mathrm{Br}} n^{-1/2},
\end{equation}

where $C^{\mathrm{Br}} = \frac{\sqrt{d}}{2}$.
\end{lemma}



\begin{proof}[Proof of Lemma \ref{lemma:hypothesis_separation_brenier}]

The interval $[1, \sqrt{\frac{R}{d^2+2d}}-1]$ is non-empty when $R\geq 4(d^2+2d)$. The Brenier embedding of the probability measure $\bs{\mu}^{(k)} = \mathcal{N}(\bs{b}^{(k)}, I_d )$ is:

$$
\forall x\in\mathbb{R}^d, \qquad \Phi^{\mathrm{Br}}(\bs{\mu}^{(k)})(x) = x^T(I_d - I_d)x + x^T\bs{b}^{(k)} = x^T \bs{b}^{(k)}
$$

We have that:

$$
\mathbb{E}\|\Phi^{\mathrm{Br}}(\bs{\mu}^{(k)})\|^4_{L^2(\rho)} = \mathbb{E} \Bigl( \int_{\mathbb{R}^d}  (b^{(k)})^T xx^tb^{(k)}\mathrm{d}\rho(x)\Bigr)^2 = \mathbb{E}\|\bs{b}^{(k)}\|^4
$$

As $\bs{b}^{(k)}\sim \mathcal{N}(0, s^{(k)}I_d)$,

$$
\mathbb{E}\|\Phi^{\mathrm{Br}}(\bs{\mu}^{(k)})\|^4_{L^2(\rho)} = (d^2+2d)(s^{(k)})^2  \leq (d^2+2d)(s^{(1)}+ \varepsilon )^2 \leq (d^2+2d)(s^{(1)} + 1)^2.
$$

Therefore, thanks to inequality \eqref{eq:s_constraint}, for $k\in \{1,2\}$, $\mathbb{E}\|\Phi^{\mathrm{Br}}(\bs{\mu}^{(k)})\|^4_{L^2(\rho)}\leq R$ and hence $\bs{\mu}^{(k)} \in \mathcal{D}(R)$. For $1\leq i\leq n$, let $f_i(x) = x^T e_i$. Then $\Phi^{\mathrm{Br}}(\bs{\mu}^{(k)}) = \sum\limits_{i=1}^d e_i^T \bs{b}^{(k)} f_i$. 

Let us compute its covariance operator
\begin{align*}
\Sigma^{(k)} &= \mathbb{E}\!\left[\Phi^{\mathrm{Br}}(\bs{\mu}^{(k)}) 
\otimes 
\Phi^{\mathrm{Br}}(\bs{\mu}^{(k)})\right]
-
\mathbb{E}\!\left[\Phi^{\mathrm{Br}}(\bs{\mu}^{(k)})\right]
\otimes 
\mathbb{E}\!\left[\Phi^{\mathrm{Br}}(\bs{\mu}^{(k)})\right]\\
&= \mathbb{E}\!\left[\sum\limits_{i=1}^d e_i^T \bs{b}^{(k)} f_i
\otimes 
\sum\limits_{j=1}^d e_j^T \bs{b}^{(k)} f_j\right]
-
\mathbb{E}\!\left[\sum\limits_{i=1}^d e_i^T \bs{b}^{(k)} f_i\right]
\otimes 
\mathbb{E}\!\left[\sum\limits_{i=1}^d e_j^T \bs{b}^{(k)} f_j\right]\\
&= \sum\limits_{i=1}^d \sum\limits_{j=1}^d e_i^T \mathbb{E}\!\left[ \bs{b}^{(k)}(\bs{b}^{(k)})^T \right]e_j f_i \otimes f_j
-
\sum\limits_{i=1}^d e_i^T \mathbb{E}\!\left[\bs{b}^{(k)}\right] f_i
\otimes 
\sum\limits_{i=1}^d  \mathbb{E}\!\left[(\bs{b}^{(k)})^T\right]e_j f_j\\
&= s^{(k)} \sum\limits_{i=1}^d \sum\limits_{j=1}^d e_i^T e_j f_i \otimes f_j\\
&= s^{(k)} \sum\limits_{i=1}^d f_i \otimes f_i\\
\end{align*}

Then, we have that:

\begin{align*}
\|\Sigma^{(1)} - \Sigma^{(2)}\|^2_{\mathrm{HS}} &= (s^{(1)} - s^{(2)})^2 \bigl\|\sum\limits_{i=1}^d f_i \otimes f_i \bigr\|^2_{\mathrm{HS}}\\
&= (s^{(1)} - s^{(2)})^2 \sum\limits_{i=1}^d \| f_i \otimes f_i \|^2_{\mathrm{HS}}\\
&= (s^{(1)} - s^{(2)})^2 \sum\limits_{i=1}^d \| f_i  \|^4_{L^2(\rho)}\\
&= (s^{(1)} - s^{(2)})^2d\\
&= d n^{-1}.
\end{align*}

Taking $C = C^{\mathrm{Br}} = \frac{\sqrt{d}}{2}$ concludes the proof.
\end{proof}


\begin{comment}
\midrule
\multirow{3}{*}{Brenier} 
  & \cite{gunsilius2022convergence} & $f$ and $g$ $s$-smooth & Smoothed empirical measure & Smoother plug-in estimator & $m^{-\frac{s}{2s+d}}$ & $m^{-\frac{s}{4s+2d}}$\\
  &  & Bandwidths assumptions &  &  & \\
  &  & for smoothing kernel &  &  & \\
\end{comment}


\begin{comment}
The idea is to solve the semi-dual optimization problem:

$$
    \varphi_{\mu} \in \argmin\limits_{\varphi \in L^2(\rho)} \int \varphi\mathrm{d}\rho +\int \varphi^*\mathrm{d}\mu,
$$

where $\varphi^*$ is the convex conjugate of $\varphi$. The map is then computed via the gradient $T_{\mu} = \nabla \varphi_{\mu}$.
\end{comment}
